Quality Matters: Evaluating Synthetic Data for Tool-Using LLMs

Training large language models (LLMs) for external tool usage is a rapidly expanding field, with recent research focusing on generating synthetic data to address the shortage of available data. However, the absence of systematic data quality checks poses complications for properly training and testing models. To that end, we propose two approaches for assessing the reliability of data for training LLMs to use external tools. The first approach uses intuitive, human-defined correctness criteria. The second approach uses a model-driven assessment with in-context evaluation. We conduct a thorough evaluation of data quality on two popular benchmarks, followed by an extrinsic evaluation that showcases the impact of data quality on model performance. Our results demonstrate that models trained on high-quality data outperform those trained on unvalidated data, even when trained with a smaller quantity of data. These findings empirically support the significance of assessing and ensuring the reliability of training data for tool-using LLMs.

==> latex/intirinsic_eval_framework.tex <==

%At first, we set out to understand what makes a data-point high quality, specifically for tool-using LLM training. Since it is impossible to track the importance of each specific data-point to the overall training process, we first seek to define a framework that evaluates data correctness for a single data-point, based on human expert assessment. Indeed, when diving deep into the dataset and manually examining several data-points, we found that the automatically generated dataset can be poorly constructed in a number of ways. We define several dimensions for error, and manually evaluate how well does the dataset do in each dimension. \sofia{add ref to section manual evaluation numbers} In this section we focus on intrinsic quality properties. We ask ourselves, using human expert assessment - what makes a data point correct and high-quality for training? 
%At first, we set out to understand what makes a data-point high quality, specifically for tool-using LLM training. When diving deep into synthetically generated datasets we found a number of possible issues, based on which we define the different types of errors.
We set out to understand what makes an instance of data high quality, specifically for training tool-using LLMs. The relevant concerns we raise for a data instance pertain to the query instruction and the API call sequence.

% We define several dimensions for error, and evaluate how well does the dataset do in each dimension.
% In the following sections we present the quality dimensions that we focus on. 
For the generated instruction itself, we check for\footnotemark: \textbf{Specificity}, \textbf{Coherence} and \textbf{Solvability}. Additionally, we check for the correctness of the ground truth API-call sequence, by measuring \textbf{Matching Parameter}, \textbf{Matching API} and \textbf{Minimal API calls}. We will provide precise definitions for each of these dimensions in following sections.

\footnotetext{We experimented with three more dimensions that were not included in the paper for several reasons. See Appendix \ref{app:additional_dimenisions} for more details.}


Tables \ref{tab:examples_instruction} and \ref{tab:examples_api} show some examples of data points with low scores for few dimension. For a more elaborate collection of  examples, see Appendix \ref{app:qualitative_examples} 
% COMMENT \shadi{TODO}. 
\input{tables/error-examples}

\subsection{Instruction Assessment}

%\zk{The definitions here are too long IMO. I propose to convert them to just a definition 1-2 lines. Then refer to an appendix that has the SOP for annotation - this will provide a more thorough an precise definition for anyone interested enough. Taking specificity as an example: ``Specificity: When an instruction requires the invocation of an API with required parameter (e.g. city name, or phone number), these details should be present in the instruction.'' It might not be very easy to understand what it means but with the SOP given in an appendix and the table showing bad examples, it should be clear enough.} \shadi{agree. changed it}

To define intrinsic quality for each data point in the dataset,  we start by looking into several dimensions of \textit{instruction correctness}. 


\paragraph{Specificity.} All required information is present for the AI assistant to fulfill user requests (e.g. city name, or phone number). No missing variables or gaps in the instructions.



\paragraph{Coherence.} Requests within an instruction are logically related. The flow of requests makes sense for a real-world use case.
 
\paragraph{Solvability.} Whether the generated instructions can be addressed by the given APIs.  

\subsection{API-call Sequence Assessment.}
Apart from the instruction itself, the other important component of the generated training set is the ground truth that is compared against during the training process. In the case of tool-using LLMs, that is the sequence of API calls that the trained model is expected to output. %Naturally, these dimensions are only meaningful for the data-points where the instruction is fully correct. \sofia{just validate this last point please}
We define four dimensions of \textit{API-call sequence correctness}: 
\paragraph{Matching Parameter.} Whether the parameter values in the API call sequence are correctly extracted or inferred from the query, and there are no missing or hallucinated parameter values.
\paragraph{Matching API Calls.} Whether the API call sequence would fully solve the user query. \footnotemark 
\footnotetext{This is somewhat similar to  \textbf{adequacy} in machine translation \cite{celikyilmaz2020evaluation}.}

\paragraph{Minimal API calls.} Whether the API call sequence solves the user query with a minimal number of calls, without unwanted API calls that are not needed to solve the query. \footnote{This dimension addresses the observed tendency of the model to sometimes invoke every API provided, potentially overlooking the given instruction. }

\subsection{Manual Annotations}

The six intrinsic criteria defined above specify the desired qualities of the data needed for training and testing tool-using LLMs. Existing datasets do not always abide by the quality criteria, especially when they are collected synthetically and do not go through a cleaning phase. We inspect such noisy data by preparing annotation guidelines with respect to the criteria, and annotating accordingly. Specifically, we annotated a sample of the training data from ToolBench \cite{qin2023toolllm} and from ToolAlpaca \cite{tang2023toolalpaca}, as well as a large portion of the ToolBench test set. We did not annotated ToolAlpaca test set since it is already human-annotated. The annotated data is used in later sections for analyses and experiments.
The inspected training data is used to assess our intrinsic evaluation metrics (Section \ref{sec_intrinsic_eval_framework}). 

\shadi{moved 4.3.1 and 4.3.2 to the appendix}
%, while the test data as well as most of the ToolBench test The annotations facilitate

%-- we have train and test sets from the same distribution but with different setup, train has api-call sequence while test does not...

\input{tables/intrinsic_metrics_subtables.tex}


==> latex/intrinsic_eval_old.tex <==
\zk{This section needs some cleanup and shortnening IMO. I suggest the following structure:\\
\begin{itemize}
    \item We need automation for the metrics
    \item First attempt is to use GPT3.5 as an annotator. Provide it the SOP and let it give ratings. We did this, the prompts are in Appendix ??
    \item For metrics A,B this didn't work well. The direct annotation task was too dificult and we replaced it with an easier task. Elaborate for each of the metrics where we used something non-direct
    \item present results. (1) present the datasets (no need to mention them before this point), (2) mention how many examples we manually annotated, (3) show results demonstrating the agreement of automated with manual, (4) show the improvement in agreement for the metrics A,B mentioned before gained by moving from a direct annotation strategy to the indirect one.
    \item If we think its worth-while, show qualitative examples (say this below, not sure if its needed, but up to you)
    \item mini-discussion related to the datasets themselves (basically Table~\ref{tab:data_statistics}). So far the focus was on the quality of the automated metrics vs manual ones. Now consider not the agreement but the actual scores for the dataset, mention the low quality of ToolAlpaca and that although ToolBench is higher quality, it still has problematic datapoints. This is basically motivation for trying to filter datasets in the first place.
\end{itemize}
}

%  \cite{DBLP:journals/corr/abs-2308-06259,DBLP:journals/corr/abs-2306-11644}

We now set out to explore automated ways to apply our evaluation framework -- it is impractical, or at the very least cost-heavy, to manually assess the training set. We provide an evaluation that shows how closely the automatic methods agree with manual annotations. Having shown a high correlation, our methods enable us to perform an intrinsic evaluation of the entire dataset.

To automate the assessment of data points, we leverage \evaluatorModel{}  as a discriminator. \shadi{TODO: we should say something about that discrimination is easier task than generation. Ori said he knows some papers that investigate this.} \ori{} Given a specific data-point -- either the instruction in the instruction assessment or the pair of (instruction, ground truth) in the ground truth assessment -- \evaluatorModel{} is prompted to evaluate  each dimension of correctness individually, using a direct question. For example, ""\sofia{add here a sentence from one of the prompts that do work using a direct questioning method}. All prompts used in this step are available in appendix \ref{sec:appendixa}. 

While automated evaluation strategies have been commonly used  \cite{DBLP:journals/corr/abs-2308-06259,DBLP:journals/corr/abs-2306-11644}, including direct questioning of the generative model and requesting ratings, we have not seen examples of the automated evaluation's results being thoroughly validated for their accuracy or alignment with human judgment. \sofia{ does this really belong here? seems more of an introduction statement. consider splitting this later on.} Our initial observations indicate potential shortcomings of the direct questioning approaches in evaluating certain dimensions, specifically for \textbf{Specificity}, \textbf{Coherence} and \textbf{Matching Parameter}. Therefore, for these dimensions specifically, we improve upon the direct questioning method and guide to perform the evaluation \evaluatorModel{} using a proxy task. We present further analysis, as well as a few examples, in Appendix \ref{sec:appendixc}. To validate the evaluation metrics, we use the manual annotation of a subset of the train set (50 examples) as described in \ref{sec:annotation_train}. Subsequently, we calculate the resulting error prediction accuracy, precision, and recall.
We now move to present the method and prompt for each correctness dimension assessment, and show the results.


\subsection{Instruction assessment}
\paragraph{Specificity.} As illustrated with examples in Appendix \ref{sec:appendixc}, GPT-3.5 struggles with identifying whether an instruction lacks specificity and does not provide real entities, as in "Fetch the top tracks of a specific artist". To address this, we  transform the direct questioning task into an NLP task, leveraging the extraction abilities of LLMs. 

We use a two-step approach, prompting the model to: 
1) Define the required parameters that the user should specify for the AI assistant to fulfill the user request
2) Extract the parameter values of the suggested parameters from step 1 out of the instruction, or use the placeholder ``\textit{\#missing}'' for parameter values not explicitly provided in the query.

We then compute a proxy specificity score $S$ using the formula: $ S = \frac{N_e}{N_t} $, 
where $N_e$ represents the number of extracted parameters, excluding instances with ``\textit{\#missing}'' values, and $N_t$ is the total number of parameters. The resulting score $S$ will range between 0 and 1, where 0 indicates low specificity, and 1 indicates high specificity. This proxy score for specificity quantifies the lack of information in the instruction regarding important attributes. We considered an instruction with $S<1$ as lacking specificity. By leveraging extraction abilities of \evaluatorModel, we observe better alignment with human evaluation. The detailed prompt is presented in Appendix \ref{sec:appendixa}.

\paragraph{Coherence.} In addressing the challenge of evaluating instruction coherence, we introduce a task similar to Next Sentence Prediction (NSP) task. We divide the given instruction into multiple sentences and direct \evaluatorModel{} to predict whether the second sentence logically follows the first one. The coherence score $C$ is defined as follows: 0 if there exists an incoherent pair and 1 otherwise.

Unlike the rating approach, our focus here is on guiding the model to assess coherence in pairs of consecutive sentences within each instruction. This targeted evaluation allows us to specifically gauge the model's ability to generate logically connected instructions. The detailed prompt for coherence evaluation is provided in Appendix \ref{app:appendixa}.

\paragraph{Solvability.} In the assessment of instruction solvability, we use the direct questioning method, instructing the model to consider the available API functions and evaluate their functionality to address the entire generated instruction. The detailed prompt for solvability evaluation is presented in Appendix \ref{sec:appendixa}. 
\input{tables/data_statistics.tex}

\subsection{API-Call Sequence Assessment}
\paragraph{Matching Parameter.} This dimension examines the accuracy of extracting and inferring parameter values from the generated instructions. Our method follows a structured approach, tasking the model with suggesting and extracting parameters from instructions, similar to the specificity task. Subsequently, we ask the \evaluatorModel{} to compare between the extracted parameter values and the API-call sequence parameters. Through this evaluation, we aim to ascertain the accuracy of the parameter values provided in the ground truth, finding instances where values are either missing or inaccurately inferred. \sofia{ did we try here to use a more direct questioning approach ("is this correct?") and failed, or did we just use the already available specificity idea? } \shadi{yes it also did not perform well.}

\paragraph{Matching API Calls.} In determining whether the API-Call sequence addresses and solves the instruction, we use a direct questioning method -- present \evaluatorModel{} with a user query alongside the list of API functions (which is considered the ground truth in the original dataset), Each API function is accompanied by its name, description, parameters, and output fields. The model is tasked with determining whether the generated API call sequence can solve the user query. 

\paragraph{Minimal API Calls.} Similar to the Matching API Calls assessment, we directly question \evaluatorModel{} to determine whether the generated API call sequence accomplishes its objective with the minimal number of calls or if redundant calls are present. 

\subsection{Validation Results}

We conduct human annotation for the six dimensions, as outlined in Section \ref{}. To validate the alignment of our methods with human evaluation, we compare our method's prediction with the human annotation and calculate accuracy (agreement), precision, recall and F1-score metrics. We treat incorrect instances as positive labels since we aim for identifying errors and filtering out incorrect samples. 
We present the results in Table \ref{tab:intrinsic_metrics}. Analyzing the results for each dimension reveals the inherent difficulty and subjectivity associated with the task of data quality assessment. Additionally, it indicates that even in a discrimination task rather than generation, \evaluatorModel{} struggles to accurately determine whether a given data sample for a tool-use task is correct.

Given that our primary objective is to identify and filter out incorrect data samples, our emphasis is on achieving high recall. This objective is largely met across most dimensions, in both datasets. In the overall assessment, which aggregates all dimensions, we observe high recall and precision, demonstrating a strong alignment with human evaluation.

\subsection{Analysis}

\label{sec:intrinsic_analysis}
\paragraph{Statistics.} Table \ref{tab:data_statistics} presents the percentage of errors in each dimension for both the ToolBench and ToolAlpaca datasets. These statistics provides insights into the quality of the data in each dataset. In the ToolBench dataset, we observe a high percentage of errors in instructions and the ground truth, in comparison to the ToolAlpaca dataset. This difference may be attributed to the complexity of the tool-use task in ToolBench, which involve training for multi-tool API call sequences. Consequently, the model is presented with a higher number of tools and APIs, resulting in longer prompts and instructed to produce complex instructions, which result in high percentage of errors. Additionally, the ground truth generation in ToolBench employs Tree of Thought, a more complex approach than Chain of Thought which is used in ToolAlpaca. This complex method produces ground truth sequences with a higher probability of errors. More importantly, the ToolBench dataset uses real-world APIs, where their documentation is not always clear, resulting in incorrect instructions and API-call sequences.

\paragraph{Qualitative Examples.} We provide 10 random samples of incorrect instructions for each dimension in Appendix \ref{app:}. \shadi{TODO: add discussion}

\paragraph{Dimensions Interactions.} \shadi{Should I show the correlation/confusion matrix between instruction correctness and ground truth correctness? or even between specificity and Parameter Matching. Or it is not reasonable to evaluate the sequence in a case of wrong instruction? \\ I have added it tell me what you think}

We explored the relationships between dimensions within the datasets. We observed that correlations between dimensions are not particularly high, which suggests that the errors we defined are distinct and not overlapping. Another aspect we explored is the effect of \textbf{Specificity} on \textbf{Matching Parameters}. As illustrated in Figure \ref{fig:spec_param_conf}, when specificity is low, a higher probability that parameter matching is low. Notably, when specificity is high, we also have good probabilty for low parameter matching, which might indicate missing parameters.

%the instruction correctness and its impact on ground truth correctness. We found that when the instruction correctness dimension indicated a lack of specificity, coherence, or solvability, it influenced the correctness of the API call sequence. In Table \ref{tab:dimension_interactions}, we showcase these findings: \input{tables/dimension_interactions.tex} \shadi{TODO: discuss briefly}



==> latex/others.tex <==


\paragraph{Specificity.} In our initial analysis of synthetic data generated using foundation models such as ChatGPT, we observed that a significant portion of instructions lacked specificity. For instance, ``\textit{Please search for all the comments made by a specific user on a Facebook page or group}''. In this example, the instruction fails to include essential details such as the user ID and the specific Facebook page or group, highlighting the model's limitation in generating precise and actionable requests. Subsequently, we observed that these vague instructions resulted in inaccurate responses, marked by missing parameters, hallucinated parameters, or incorrect alignment of the LLM with a reasonable user's request. 


\paragraph{Coherence.} We focus on the coherence of instructions and the generative model's ability to seamlessly convey multiple requests for multi-instructions. For example, %picking two different APIs and creating a single request that uses both of them, tends to create a single instruction that illogically connects between two very different instructions -- in a way that does not represent an instruction that a reasonable user would ask from an automated system. For example, 
``\textit{I want to impress my friends with some hilarious jokes. Can you fetch some jokes related to 'sports'? Also, fetch the exchange rate from GBP to EUR.}'' In this generated instruction, two distinct and unrelated tasks are combined, presenting a scenario that may not align with real-world contexts. This lack of coherence may result in demonstrations that deviate from the distribution observed in real-world human-generated instructions. 
%Moreover, these instructions, which are unrelated to each other, and given the fully automated judgement system that trains the model, tend to result in a training process that ignores mistakes such as only generating the response to one of the requests. \sofia{do we have a good example for this?? I feel we need to explain logically why is coherence important} \shadi{I didn't notice this, isn't the next reason+not representing real-wolrd instructions enough?} \sofia{ re the automated judgement system - does it judge all parts well? didn't we have an issue with it only judging the first task when tasks are unrelated? I just feel like a very easy dismissal of coherence would be "it can be okay to ask for two unrelated things at ones there's nothing wrong with having such examples", and I feel we need to defend our statement that it is important with more than just a hunch + extrinsic evaluation later}
Another important factor, is that tool-using LLM that needs to use more than one API call might need to also perform a calculation or a logical leap given the results of the first call in order to invoke the second one. For example, the following instruction: "I want to find a specific movie but I only remember the title 'Inception'. Can you help me search for the movie 'Inception' and provide me with its details, including the genre, runtime, IMDb rating, and streaming availability?" might require two API calls -- one to find the imdb id of the movie 'Inception' using a search-API, and another to fetch the necessary details about it, using the fetched information within the call. When the training data consists of data points that mostly have incoherent calls that are unrelated to each other, the model will never have a chance to learn this complexity of instructions that are interdependent. 
\sofia{coherence is way too long. we need to discuss maybe remove or move some of the justifications here to footnotes}

\paragraph{Solvability.} In the context of instruction generation, solvability refers to whether the generated instructions can be addressed by the given APIs. Since the instructions are generated automatically, usually given the API description as an input, the generation can sometimes create an instruction that does not fit the intended API - or indeed is impossible to solve altogether. Including unsolvable examples in the training set, which can only result in a wrong API-call sequence, can negatively impact the training process of the LLM. 


==> latex/related_old.tex <==
\shadi{We need to shorten related work section}
\subsection{Tool usage}
Tool learning \cite{qin2023tool} is a recent area of research aiming to enhance the capabilities of LLMs by allowing them to invoke tools, helping them to overcome their weaknesses, e.g. 
retrieval for making use of recent information, or a calculator for mathematical operations, or allowing them to act in the real world \zk{note: consider adding citations for these use cases}. 

\sofia{we should shorten this, as we say: "our focus is more towards the element of data collection as this relates most closely to our paper"... - we can cite the relevant papers and say something like "a lot of recent activity has been focused on the different aspects of methods for training tool-using LLMs, challange 1 [cites], + two sentences. ..." }
There main challenges in teaching an LLM to invoke tools can be, in high level, partitioned to the following: Tool selection, tool usage, and planning (for cases where multiple tools are required). For each challenge, papers devised both training methods, inference methods and data collection methods. While we briefly review all of these, our focus is more towards the element of data collection as this relates most closely to our paper.

For tool selection, the challenge is teaching the LLM to know when a tool should be invoked, and if one is needed, which tool to select. In \cite{schick2024toolformer}, the authors provide a self-supervised way to teach the LLM to invoke a pre-defined small set of tools. Here, there is not much need for collecting or generating specialized data, but as a result the technique is suited for commonly used tools such as calculator, calendar, information retrieval, and would likely require a new data collection or generation process for more specialized tools. In Gorilla LLM \cite{patil2023gorilla}, the authors highlight the additional challenge of tool usage when the number of tools is large, e.g. in the 1000s. They propose to add a retrieval component to the LLM, meaning that given a request, this retrieval will choose an appropriate tool (or a handful 
of tools) and add its definition to the prompt of the LLM. The LLM can than choose whether to invoke this tool. In addition to having a retrieval component, it was shown to be helpful to finetune 
the LLM for tool usage. In particular, this finetuning process was shown to be generalizable to other tools, meaning one set of tools was used when fine tuning, and a different set when testing. 
A similar conclusion motivating a finetuning process was reached in other papers 
\cite{qin2023toolllm, li2023api,DBLP:journals/corr/abs-2306-05301}. Note that for finetuning, one requires data; this data is generated in \cite{patil2023gorilla} by prompting an LLM to provide an instruction matching a given API. For the challenge of deciding whether a tool should be invoked, \cite{huang2023metatool} provide a synthetic dataset based on the tools of openAI plugin list, they generate multiple instruction for each tool, as well as instructions that do not require the use of any tool. They ensure diversity by generating instructions of different tones and sentiment, and ensure quality of individual examples via human inspection. 


For tool usage, the challenge is that once the LLM made the decision to invoke a certain tool, it should be able to do so correctly, meaning use the correct tool and parameter names, extract the right parameter values from the request and if needed (and allowed), as the user for required and missing parameters. It is possible to teach the LLM to invoke the tools correctly via fine-tuning as is done, e.g. in \cite{schick2024toolformer, zhuang2024toolqa, yao2023react}. However, when the number of tools increase this becomes challenging as it requires more data and a heavier reliance on the fine-tuning process. Moreover, it is not possible for such systems to handle new tools at inference time. For such cases, a straightforward approach would be to provide the complete definition of a tool to the prompt of the LLM (this was done e.g. in \cite{patil2023gorilla}). The limitation here is that when presenting more than one choice, the prompt can become too long. A mitigation for this issue is given by \cite{hao2024toolkengpt} that provide a system where only once the tool is selected by the LLM (by generating a specific token), the prompt is modified to include the full instructions for the tool.
\sofia{if it's outside score - let's edit it out!!}
The third challenge of planning is mosly outside the scope of our paper. Here, the main approaches are done by modifying the inference. In ReAct \cite{yao2023react} the authors propose to let the LLM explain its action in natural language, then act. In the context of tool learning act means invoke a tool. In Toolformer \cite{schick2024toolformer}, the authors propose a tree traversal approach for inference, where the correct path for inference, meaning sequence of tool invocation, is planned, validated and if needed backtracked. This approach leads to higher quality results even when compared to selecting the best out of multiple invocations of simpler approaches (when making the runtime equivalent). From the lens of data generation, the requirement here is to have example instructions that require invoking more than a single tool. To this end in Toolformer \cite{schick2024toolformer}, a handful of tools are selected at random either from the entire pool of APIs or from a certain category of APIs. The latter ensures the selected tools are more likely to be required in a single instruction. \cite{huang2023metatool} choose random tool pairs from a pool of commonly used tools, thus increasing the chance of it being possible to build an instruction requiring both tools.

We mention here a few more notable works that created synthetic data for tool learning. It is shown (e.g. \cite{xu2023tool}) that open source LLMs exhibit sub-optimal performance when tested on tool learning tasks, both with zero shot and few-shot settings. This is in contrast to close sourced LLMs that are conjectured to have some fine-tuning done aimed for tool usage. With this in mind, there is a clear need for training sets to teach LLMs to invoke tools correctly. Tool LLM \cite{qin2023toolllm} generate data using ChatGPT (gpt-3.5-turbo-16k). They draw one or a handful of tools from a pool of 16000 real tools (from RapidAPI) using several sampling methods, controlling how related these tools are, and prompt ChatGPT to build an instruction that would require invoking these tools, as well as a solution path. The test set used is a random sample of the training set, though the testing procedure does not rely on a ground truth answer, rather on an evaluation of the response by a strong LLM (e.g. GPT4). In API bank \cite{li2023api}, the authors aim to focus on APIs with clean and uniform documentation, hence they generate not only the training data but the APIs + their documnetation. They use GPT4 to generate the API documentation, given one or a handful of APIs they invoke GPT4 to generate an instruction and ground truth response, and finally they have a step of validating the quality of the generated example. We note that this last step is not fully documented in the paper, so we were not able to compare it to the quality validations proposed here. The test set provided by  \cite{li2023api} is smaller but of higher quality; it is generated and validated by humans. toolAlpaca \cite{DBLP:journals/corr/abs-2306-05301} use a similar approach to  \cite{li2023api} in that they have an LLM generate APIs. Here, the focus is on instruction that require a single API, and the data generation for training data is done by invoking an LLM (GPT4) to create an instruction and solution given an API. The test set is prepared with human assistance to ensure quality. \cite{yang2024gpt4tools} focus on tools related to image processing. Given a tool and an image they invoke an LLM to generate an instruction that will require applying the tool to that image. They post-process the generated instructions to remove near-duplicates and add instructions similar to those generated that do not require invoking a tool. ToolQA \cite{zhuang2024toolqa} focus on tools for question answering in multiple domains. They generate data based on manually built templates. This ensures high quality data but requires intensive labor for generating diverse templates.

\zk{Do we need to mention T-eval \cite{chen2023t}? If so, how does it relate to our work? Do we use it for evaluation? If not we should explain why, if yes we should mention it. } {\shadi{We do not use it. I think we should only mention it, the paper came out in the middle of our work 3 months ago}}


% a way to introduce tool usage in a pre-training procedure of an LLM, meaning allow a self supervised training method for 
 
%  Tool LLM \cite{qin2023toolllm}, Gorilla \cite{patil2023gorilla}, toolformer \cite{schick2024toolformer}... 
%  API bank \cite{li2023api}, toolAlpaca \cite{DBLP:journals/corr/abs-2306-05301}

% ToolQA \cite{zhuang2024toolqa} focus on QA tools. 
% MetaTool \cite{huang2023metatool} a benchmark for whether to use tools. 


\subsection{Reducing dataset size}
A recent line of work shows that s small but high quality dataset can be highly effective for fine-training a 1.3B model that surpress the quality of 7B models. 
Phi \cite{gunasekar2023textbooks} considered code generation, and showed that highly a few examples that are highly diverse are sufficient to reach high code generation quality. This was later expanded in Phi 1.5, where an additional NLP dataset for commonsense reasoning was again sufficient for a small model to reach very high quality results. 
In Lima \cite{zhou2024lima}, the authors show that as few as 1k high quality examples can be sufficient for training an instruction following model. 

\zk{these papers aren't related to reducing dataset size. We can (probably should) mention them as data generation papers that do not relate to tool usage}
WizardLM \cite{xu2023wizardlm} is a method for generating synthetic data for instruction finetuning. 
Instead of generating data directly via an LLM, which results in low quality examples, they run the generation in multiple steps, continuously evolving the quality and diversity of the results. 
Humpback \cite{li2023self} is another system for generating synthetic data for instruction finetuning. 
They combined the idea of evolving instructions together with filtering to remove bad examples from the dataset while generating more diverse and high quality examples. 

\ori{add t-eval sentence}

==> tables/dimension_interactions.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|c|}
\hline
\textbf{Instructions} & \textbf{Incorrect Ground Truth} \\
\hline
Specific & 72.8\% \\
Unspecific & 80.6\% \\
\hline
Coherent & 73.8\% \\
Incoherent & 76.5\% \\
\hline
Solvable & 71.9\% \\
Unsolvable & 85.7\% \\
\hline
\end{tabular}
\caption{Impact of instruction correctness on ground truth correctness.}
\label{tab:dimension_interactions}
\end{table}

==> tables/extrinsic_results_old.tex <==
\renewcommand{\arraystretch}{1.2} 
\begin{table*}[h]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\textbf{\small Model} & \textbf{\small I1\_inst} & \textbf{\small I1\_tool} & \textbf{\small I1\_cat} & \textbf{\small I2\_inst} & \textbf{\small I2\_cat} & \textbf{\small I3\_inst} & \textbf{\small All Samples}  \\ \hline
\small Low ICE & $0.14$ & $0.25$ & $0.23$ & $0.23$ & $0.12$ & $0.32$ & $0.20$  \\ \hline
\small Random & $0.39$ & $0.29$ & $0.27$ & $0.28$ & $0.31$ & $0.47$ & $0.34$  \\ \hline
\small MED ICE & $0.42$ & $0.29$ & $0.26$ & $0.42$ & $0.34$ & $0.50$ & $0.37$  \\ \hline
\small HIGH ICE & $0.29$ & $0.42$ & $0.34$ & $0.44$ & $0.38$ & $0.62$ & $0.40$  \\ \hline
\small HIGH INST\_GT & $0.35$ & $0.54$ & $0.35$ & $0.57$ & $0.42$ & $0.56$ & $0.45$ \\ \hline
\small HIGH INST & $0.40$ & $0.46$ & $0.34$ & $0.62$ & $0.42$ & $0.71$ & $0.46$  \\ \hline
\small ToolLLaMA & $0.36$ & $0.46$ & $0.32$ & $0.65$ & $0.45$ & $0.41$ & $0.42$  \\ \hline

\end{tabular}
\caption{Evaluation Results}
\label{tab:evaluation-results}
\end{table*}


==> tables/ice_instrinsic_corr_1.tex <==

\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|c|c|}
\hline
\multirow{2}{*}{\textbf{   Dataset}} & \multicolumn{2}{c|}{\textbf{Mean ICE Scores}} \\ 
\cline{2-3}
                 & \textbf{\small Correct} & \textbf{\small Incorrect} \\ \hline
ToolBench & 0.330 ±0.24 & 0.398 ±0.23 \\ \hline
ToolAlpaca & 0.573 ±0.21 & 0.607 ±0.13 \\ \hline
\end{tabular}
\caption{Mean and standard deviation of ICE scores by overall correctness and dataset}
\label{tab:ice_scores_stats}
\end{table}

==> tables/ice_instrinsic_corr_2.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|c|c|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{ Overall Correctness (\%)}} \\
\cline{2-3}
&\textbf{Low ICE }&\textbf{High ICE }\\ \hline
ToolBench & 13.83 & 20.74 \\ \hline
ToolAlpaca & 39.50 & 60.26  \\ \hline
\end{tabular}
\caption{Overall correctness percentage for ICE score groups by dataset.}
\label{tab:mean_correctness_ice}
\end{table}

==> tables/intrinsic_groundtruth.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.3} % Adjust the vertical space between rows
\setlength{\tabcolsep}{7pt} % Adjust the horizontal space between columns
\begin{tabular}{lcccc}
\hline
\textbf{Metric} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hline
Parameter Correctness & 0.70 & 0.63 & 0.92 & 0.74 \\
API Matching & 0.78 & 0.64 & 0.60 & 0.62 \\
Minimal API Call & 0.76 & 0.95 & 0.63 & 0.76 \\
\textbf{Overall} & \textbf{0.82} & \textbf{0.83} & \textbf{0.94} & \textbf{0.88} \\
\hline
\end{tabular}
\caption{Evaluation results for Ground Truth Correctness within each dimension and overall, considering a holistic assessment across the three dimensions.}
\label{tab:evaluation_metrics_another}
\end{table*}


==> tables/intrinsic_instruction.tex <==
\renewcommand{\arraystretch}{1.3} % Adjust the vertical space between rows
\setlength{\tabcolsep}{7pt} % Adjust the horizontal space between columns
\begin{table*}[t]
\centering
\begin{tabular}{lcccc}
\hline
\textbf{Dimension} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hline
Specificity & 0.74 & 0.70 & 0.84 & 0.76  \\
Coherence & 0.80 & 0.56 & 0.75 & 0.64  \\
Solvable & 0.90 & 0.70 & 0.78 & 0.73  \\
\textbf{Overall} & \textbf{0.86} & \textbf{0.89} & \textbf{0.92} & \textbf{0.91}  \\
\hline
\end{tabular}
\caption{Evaluation results of instruction correctness methods within each dimension and overall. The overall correctness is determined by considering the correctness in each of these dimensions.}
\label{tab:instrinsic_instruction}
\end{table*}

==> tables/intrinsic_metrics_alpaca.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.3} % Adjust the vertical space between rows
\setlength{\tabcolsep}{7pt} % Adjust the horizontal space between columns
\begin{tabular}{lccccc}
\hline
\textbf{} & \textbf{Dimension} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{Instruction}}} & Specificity & 0.88 & 0.75 & 0.86 & 0.80 \\
& Coherence & 0.98 & 0.5 & 1.00 & 0.66 \\
& Solvable & 0.92 & 0.75 & 0.50 & 0.60 \\
& \textbf{Instruction Correctness} & \textbf{0.86} & \textbf{0.80} & \textbf{0.84} & \textbf{0.82} \\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{API-Calls}}} & Parameter Correctness & 0.76 & 0.74 & 0.80 & 0.77 \\
& API Matching & 0.88 & 0.80 & 0.50 & 0.62 \\
& Minimal API Call & 0.86 & 0.88 & 0.57 & 0.70 \\
& \textbf{API-Calls Correctness} & \textbf{0.76} & \textbf{0.75} & \textbf{0.85} & \textbf{0.80} \\
\hline
& \textbf{Overall Correctness} & \textbf{0.76} & \textbf{0.74} & \textbf{0.90} & \textbf{0.81} \\
\hline
\end{tabular}
\caption{Updated validation results of Instruction Correctness and API-Call Sequence Correctness within each dimension and overall. The overall correctness is determined by considering the correctness in each of these dimensions.}
\label{tab:intrinsic_metrics}
\end{table*}


==> tables/intrinsic_metrics_bench.tex <==

\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.3} % Adjust the vertical space between rows
\setlength{\tabcolsep}{7pt} % Adjust the horizontal space between columns
\begin{tabular}{lccccc}
\hline
\textbf{} & \textbf{Dimension} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{Instruction}}} & Specificity & 0.74 & 0.70 & 0.84 & 0.76 \\
& Coherence & 0.80 & 0.56 & 0.75 & 0.64 \\
& Solvable & 0.90 & 0.70 & 0.78 & 0.73 \\
    & \textbf{Instruction Correctness} & \textbf{0.86} & \textbf{0.80} & \textbf{0.84} & \textbf{0.82} \\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{API-Calls}}} & Parameter Correctness & 0.70 & 0.63 & 0.92 & 0.74 \\
& API Matching & 0.78 & 0.64 & 0.60 & 0.62 \\
& Minimal API Call & 0.76 & 0.95 & 0.63 & 0.76 \\
& \textbf{API-Calls Correctness} & \textbf{0.82} & \textbf{0.83} & \textbf{0.94} & \textbf{0.88} \\
\hline

\end{tabular}
\caption{Validation results of Instruction Correctness and API-Call Sequence Correctness within each dimension and overall. The overall correctness is determined by considering the correctness in each of these dimensions.  }
\label{tab:intrinsic_metrics}
\end{table*}
